Morphology of small snarks

The aim of this paper is to classify all snarks up to order $36$ and explain the reasons of their uncolourability. The crucial part of our approach is a computer-assisted structural analysis of cyclically $5$-connected critical snarks, which is justified by the fact that every other snark can be constructed from them by a series of simple operations while preserving uncolourability. Our results reveal that most of the analysed snarks are built up from pieces of the Petersen graph and can be naturally distributed into a small number of classes having the same reason for uncolourability. This sheds new light on the structure of all small snarks. Based on our analysis, we generalise certain individual snarks to infinite families and identify a rich family of cyclically $5$-connected critical snarks.

==> pozn.tex <==
the flow through exactly one of its connectors $I$ and $O$
- vs I, O / I or O

Then we add one vertex $v$ incident with the semiedges $r_1$, $r_2$

We prove that for each colouring $\phi$ of $H$, the number of connectors of $H$ having nonzero flow is even. (are even? - asi skôr nie)

Ann. N. Y. Acad. Sci. je to správna skratka?

------------------

Journal of Combinatorial Theory, Series B .> J. Combin. Theory Ser. B
Electronic Notes in Discrete Mathematics -> Electron. Notes Discrete Math.

------------------
Dangling edge - one free end and that end is semiedge
